End-to-End Learning of OFDM Waveforms with PAPR and ACLR Constraints

Orthogonal frequency-division multiplexing (OFDM) is widely used in modern wireless networks thanks to its efficient handling of multipath environment. However, it suffers from a poor peak-to-average power ratio (PAPR) which requires a large power backoff, degrading the power amplifier (PA) efficiency. In this work, we propose to use a neural network (NN) at the transmitter to learn a high-dimensional modulation scheme allowing to control the PAPR and adjacent channel leakage ratio (ACLR). On the receiver side, a NN-based receiver is implemented to carry out demapping of the transmitted bits. The two NNs operate on top of OFDM, and are jointly optimized in and end-to-end manner using a training algorithm that enforces constraints on the PAPR and ACLR. Simulation results show that the learned waveforms enable higher information rates than a tone reservation baseline, while satisfying predefined PAPR and ACLR targets.

==> V1/abbreviations.tex <==
\newacronym{3GPP}{3GPP}{3rd Generation Partnership Project}
\newacronym{ACM}{ACM}{adaptive coding and modulation}
\newacronym{ACLR}{ACLR}{adjacent channel leakage ratio}
\newacronym{ADC}{ADC}{analog-to-digital conversion}
\newacronym{AGC}{AGC}{automatic gain control}
\newacronym{AWGN}{AWGN}{additive white Gaussian noise}
\newacronym{BER}{BER}{bit error rate}
\newacronym{BS}{BS}{base station}
\newacronym{BLER}{BLER}{block error rate}
\newacronym{BCE}{BCE}{binary cross-entropy}
\newacronym{BICM}{BICM}{bit-interleaved coded modulation}
\newacronym{BMD}{BMD}{bit-metric decoding}
\newacronym{BP}{BP}{backpropagation}
\newacronym{BPTT}{BPTT}{backpropagation through time}
\newacronym{CE}{CE}{cross-entropy}
\newacronym{CFO}{CFO}{carrier frequency offset}
\newacronym{CNN}{CNN}{convolutional neural network}
\newacronym{CCDF}{CCDF}{complementary cumulative distribution function}
\newacronym{CSI}{CSI}{channel state information}
\newacronym{DAC}{DAC}{digital-to-analog conversion}
\newacronym{DPD}{DPD}{digital pre-distortion}
\newacronym{DL}{DL}{deep learning}
\newacronym{DFT}{DFT}{discrete Fourier transform}
\newacronym{ELU}{ELU}{exponential linear unit}
\newacronym{FFT}{FFT}{fast Fourier transform}
\newacronym{GAN}{GAN}{generative adversarial network}
\newacronym{GRU}{GRU}{gated recurrent unit}
\newacronym{iid}{i.i.d.\@}{independent and identically distributed}
\newacronym{IFFT}{IFFT}{inverse fast Fourier transform}
\newacronym{KL}{KL}{Kullback-Leibler}
\newacronym{LLR}{LLR}{log-likelihood ratio}
\newacronym{LSTM}{LSTM}{long short-term memory}
\newacronym{LDPC}{LDPC}{low-density parity-check}
\newacronym{LMMSE}{LMMSE}{linear minimum mean squared error}
\newacronym{MDP}{MDP}{Markov decision process}
\newacronym{ML}{ML}{machine learning}
\newacronym{MLP}{MLP}{multilayer perceptron}
\newacronym{MIMO}{MIMO}{multiple-input multiple-output}
\newacronym{MU-MIMO}{MU-MIMO}{multi-user multiple-input multiple-output}
\newacronym{MU}{MU}{multi-user}
\newacronym{MSE}{MSE}{mean squared error}
\newacronym{NN}{NN}{neural network}
\newacronym{NR}{NR}{new radio}
\newacronym{NLOS}{NLOS}{non-line of sight}
\newacronym{OFDM}{OFDM}{orthogonal frequency-division multiplexing}
\newacronym{pdf}{pdf}{probability density function}
\newacronym{pmf}{pmf}{probability mass function}
\newacronym{PA}{PA}{power amplifier}
\newacronym{PAPR}{PAPR}{peak-to-average power ratio}
\newacronym{PSD}{PSD}{power spectral density}
\newacronym{PRT}{PRT}{peak reduction tone}
\newacronym{QPSK}{QPSK}{quadrature phase-shift keying}
\newacronym{QAM}{QAM}{quadrature amplitude modulation}
\newacronym{PSNR}{PSNR}{Peak Signal to Noise Ratio}
\newacronym{RBF}{RBF}{Rayleigh block-fading}
\newacronym{RB}{RB}{resource block}
\newacronym{RE}{RE}{resource element}
\newacronym{RG}{RG}{resource grid\newacronym{RE}{RE}{resource element}}
\newacronym{ReLU}{ReLU}{rectified linear unit}
\newacronym{RTN}{RTN}{radio transformer network}
\newacronym{RL}{RL}{reinforcement learning}
\newacronym{RNN}{RNN}{recurrent neural network}
\newacronym{SFO}{SFO}{sampling frequency offset}
\newacronym{SER}{SER}{symbol error rate}
\newacronym{SNR}{SNR}{signal-to-noise ratio}
\newacronym{SINR}{SINR}{signal-to-interference-plus-noise ratio}
\newacronym{SGD}{SGD}{stochastic gradient descent}
\newacronym{SISO}{SISO}{single-input single-output}
\newacronym{SIMO}{SIMO}{single-input multiple-output}
\newacronym{SU}{SU}{single-user}
\newacronym{TDD}{TDD}{time-division duplexing}
\newacronym{TR}{TR}{tone reservation}
\newacronym{UE}{UE}{user equipment}
\newacronym{UMi}{UMi}{urban microcell}
\newacronym{wrt}{w.r.t.\@}{with respect to}



==> V1/macros.tex <==
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\vecs}[1]{\boldsymbol{#1}}

\newcommand{\av}{\vec{a}}
\newcommand{\bv}{\vec{b}}
\newcommand{\cv}{\vec{c}}
\newcommand{\dv}{\vec{d}}
\newcommand{\ev}{\vec{e}}
\newcommand{\fv}{\vec{f}}
\newcommand{\gv}{\vec{g}}
\newcommand{\hv}{\vec{h}}
\newcommand{\iv}{\vec{i}}
\newcommand{\jv}{\vec{j}}
\newcommand{\kv}{\vec{k}}
\newcommand{\lv}{\vec{l}}
\newcommand{\mv}{\vec{m}}
\newcommand{\nv}{\vec{n}}
\newcommand{\ov}{\vec{o}}
\newcommand{\pv}{\vec{p}}
\newcommand{\qv}{\vec{q}}
\newcommand{\rv}{\vec{r}}
\newcommand{\sv}{\vec{s}}
\newcommand{\tv}{\vec{t}}
\newcommand{\uv}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\wv}{\vec{w}}
\newcommand{\xv}{\vec{x}}
\newcommand{\yv}{\vec{y}}
\newcommand{\zv}{\vec{z}}
\newcommand{\zerov}{\vec{0}}
\newcommand{\onev}{\vec{1}}
\newcommand{\alphav}{\vecs{\alpha}}
\newcommand{\betav}{\vecs{\beta}}
\newcommand{\varepsilonv}{\vecs{\varepsilon}}
\newcommand{\gammav}{\vecs{\gamma}}
\newcommand{\lambdav}{\vecs{\lambda}}
\newcommand{\muv}{\vecs{\mu}}
\newcommand{\omegav}{\vecs{\omega}}
\newcommand{\sigmav}{\vecs{\sigma}}
\newcommand{\thetav}{\vecs{\theta}}
\newcommand{\psiv}{\vecs{\psi}}
\newcommand{\epsilonv}{\vecs{\epsilon}}


% Matrices
\newcommand{\Am}{\vec{A}}
\newcommand{\Bm}{\vec{B}}
\newcommand{\Cm}{\vec{C}}
\newcommand{\Dm}{\vec{D}}
\newcommand{\Em}{\vec{E}}
\newcommand{\Fm}{\vec{F}}
\newcommand{\Gm}{\vec{G}}
\newcommand{\Hm}{\vec{H}}
\newcommand{\Id}{\vec{I}}
%\newcommand{\Id}{\mathds{1}}
\newcommand{\Jm}{\vec{J}}
\newcommand{\Km}{\vec{K}}
\newcommand{\Lm}{\vec{L}}
\newcommand{\Mm}{\vec{M}}
\newcommand{\Nm}{\vec{N}}
\newcommand{\Om}{\vec{O}}
\newcommand{\Pm}{\vec{P}}
\newcommand{\Qm}{\vec{Q}}
\newcommand{\Rm}{\vec{R}}
\newcommand{\Sm}{\vec{S}}
\newcommand{\Tm}{\vec{T}}
\newcommand{\Um}{\vec{U}}
\newcommand{\Vm}{\vec{V}}
\newcommand{\Wm}{\vec{W}}
\newcommand{\Xm}{\vec{X}}
\newcommand{\Ym}{\vec{Y}}
\newcommand{\Zm}{\vec{Z}}
\newcommand{\Lambdam}{\vecs{\Lambda}}
\newcommand{\Sigmam}{\vecs{\Sigma}}
\newcommand{\Omegam}{\vecs{\Omega}}
\newcommand{\Pim}{\vecs{\Pi}}
\newcommand{\Psim}{\vecs{\Psi}}
\newcommand{\Xim}{\vecs{\Xi}}
\newcommand{\Gammam}{\vecs{\Gamma}}

% Calligraphic
\newcommand{\Ac}{{\cal A}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Gc}{{\cal G}}
\newcommand{\Hc}{{\cal H}}
\newcommand{\Ic}{{\cal I}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Kc}{{\cal K}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Oc}{{\cal O}}
\newcommand{\Pc}{{\cal P}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Sc}{{\cal S}}
\newcommand{\Tc}{{\cal T}}
\newcommand{\Uc}{{\cal U}}
\newcommand{\Wc}{{\cal W}}
\newcommand{\Vc}{{\cal V}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Zc}{{\cal Z}}

% Number sets
\newcommand{\CC}{\mathbb{C}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\OO}{\mathbb{O}}

% Mixed symbols
\newcommand{\htp}{^{\mathsf{H}}}
\newcommand{\tp}{^{\mathsf{T}}}

% Brackets
\newcommand{\LB}{\left(}
\newcommand{\RB}{\right)}
\newcommand{\LP}{\left\{}
\newcommand{\RP}{\right\}}
\newcommand{\LSB}{\left[}
\newcommand{\RSB}{\right]}

% Useful functions
\renewcommand{\ln}[1]{\mathop{\mathrm{ln}}\LB #1\RB}
\renewcommand{\log}[1]{\mathop{\mathrm{log}}\LB #1\RB}
\renewcommand{\exp}[1]{\mathop{\mathrm{exp}}\LB #1\RB}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\diagpart}{\mathop{\mathrm{diag\_part}}}

% Expectation, Variance, etc
\newcommand{\EE}{{\mathbb{E}}}
\newcommand{\VV}{{\mathbb{V}}}
\newcommand{\Expect}[2]{\EE_{#1}\LSB #2\RSB}
\newcommand{\indicator}[1]{\mathbbm{1}\LB#1\RB}

\newcommand{\ReLU}{\mathop{\mathrm{ReLU}}}
\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\sigmoid}{\mathop{\mathrm{sigmoid}}}
\newcommand{\softmax}{\mathop{\mathrm{softmax}}}

% argmax, argmin
 \newcommand{\argmax}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{max}}\;}
 \newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{min}}\;}

%hats
\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}

\newcommand{\triplehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\doublehat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\doublehat{#1}}}}

% Beamer
\newcommand{\slide}[2]{\begin{frame}\frametitle{#1} #2 \end{frame}}

\newcommand{\titleslide}{\begin{frame}\titlepage \end{frame}}
\newcommand{\tocslide}{\begin{frame}\frametitle{Overview}\tableofcontents \end{frame}}

\newcommand{\textslide}[1]{\slide{}{
\vspace{30pt}
\begin{shaded}
\begin{center}
{\huge #1}
\end{center}
\end{shaded}
}}

\newcommand{\referenceslide}{\begin{frame}[allowframebreaks]{References}
\begin{footnotesize}
 \bibliographystyle{IEEEtranSA}
 \bibliography{../latex_common/IEEEabrv,../latex_common/refs}
\end{footnotesize}
\end{frame}}

% Norm
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\newcommand\abs[1]{\mathopen|#1\mathclose|}

==> V1/sections/abstract.tex <==
\begin{abstract}

\Gls{OFDM} is widely used in modern wireless networks thanks to its efficient handling of multipath environment.
%However, the next generation of radio systems will need to satisfy new \gls{PAPR} and \gls{ACLR} requirements.
However, it suffers from a poor \gls{PAPR} which requires a large power backoff, degrading the \gls{PA} efficiency.
In this work, we propose to use a \gls{NN} at the transmitter to learn a high-dimensional modulation scheme allowing to control the \gls{PAPR} and \gls{ACLR}. On the receiver side, a \gls{NN}-based receiver is implemented to carry out demapping of the transmitted bits.
The two \glspl{NN} operate on top of \gls{OFDM}, and are jointly optimized in and end-to-end manner using a training algorithm that enforces constraints on the \gls{PAPR} and \gls{ACLR}.
%In this work, we present an original optimization procedure, along with \gls{NN}-based transmitter and receiver architectures, that allows the emergence of new high-dimensional modulations and corresponding demappers.
%The first step is to convert the information rate of the transmission, as well as the \gls{ACLR} and \gls{PAPR} of the generated signals, to loss functions that can be minimized.
%Training of the end-to-end systems is performed using the augmented Lagrangian method, where all relevant metrics are converted to loss functions that are iteratively minimized.
Simulation results show that the learned waveforms enable higher information rates than a tone reservation baseline, while satisfying predefined \gls{PAPR} and \gls{ACLR} targets.
%Simulation results show that the proposed systems are able to achieve lower \gls{PAPR} and higher rates than a baseline using \glspl{PRT}, while satisfying \gls{ACLR} targets
\end{abstract}



==> V1/sections/autoencoder.tex <==
\section{Learning a high-dimensional modulations}
\label{sec:autoenoder}

\subsection{Problem formulation}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.42\textwidth]{figs/E2E_system.png}
    \caption{Trainable system, where grayed blocks represent trainable components.}
    \label{fig:system2}
\end{figure}


The proposed end-to-end system architecture  is depicted in Fig.~\ref{fig:system2}.
It is composed of a neural tranmsitter and neural receiver,  having trainable parameters respectively denoted by $\thetav$ and $\psiv$ and that operate on top of OFDM.
In the following, the end-to-end system will be referred to as "E2E" system for brevity.
We aim at optimizing the E2E system to design a high-dimensional modulation and a corresponding detector that maximize an achievable rate under \gls{PAPR} and \gls{ACLR} constraints.
The considered rate is \cite{pilotless20}
\begin{align}
\label{eq:rate0}
C(\thetav, \psiv) & = \frac{1}{N}\sum_{n=0}^{N-1}\sum_{k=0}^{K-1}I\left( b_{n,k}; \yv \right | \thetav)\\
& - \frac{1}{N}\sum_{n=0}^{N-1}\sum_{k=0}^{K-1}\EE_{\yv}\left[\text{D}_\text{KL} \left( P (b_{n,k}|\yv)|| \widehat{P}_{\psiv}(b_{n,k}| \yv ) \right) \right] \nonumber
\end{align}
%
which was shown to be achievable assuming a bit metric decoder \cite{bocherer2017achievable}.
%The derivation of \eqref{eq:rate0} can be carried out using the random coding argument method, as is done in \cite{pilotless20}.
The first term in \eqref{eq:rate0} is the mutual information between $b_{n,k}$ and $\yv$, and corresponds to an achievable information rate assuming an ideal receiver. 
The second term in \eqref{eq:rate0} is the KL-divergence between the true posterior probability $P (b_{n,k}|\yv)$ and the one estimated by our \gls{NN}-receiver $\widehat{P}_{\psiv}(b_{n,k}| \yv )$. 
Such probabilities can be obtained from the \gls{LLR} corresponding to the bit $b_{n,k}$, which is defined by
\begin{equation}
\text{LLR}(n,k) \coloneqq \text{ln} \left( \frac{\widehat{P}_{\psiv}(b_{n,k} = 1| \yv ) }{\widehat{P}_{\psiv}(b_{n,k} = 0| \yv ) } \right).
\end{equation}
%Such probabilities can be obtained by applying the sigmoid function to the predicted \glspl{LLR}, i.e., $\widehat{P}_{\psiv}(b_{n,k} = 1| \yv ) = \text{sigmoid}(\text{LLR}(n,k))$.
Intuitively, the KL-divergence term corresponds in \eqref{eq:rate0} to a rate loss due to an imperfect receiver.


Let us denote by $\gamma_{\text{peak}}$ the targeted PAPR and by $\beta_{\text{leak}}$ the targeted ACLR.
In the E2E system, both quantities depend on the trainable parameters of the neural transmitter.
Maximizing the rate under these constraints can be formulated as the following optimization problem :
%
\begin{subequations}
\label{eq:rate}
 \begin{align}
\underset{\thetav, \psiv}{\text{maximize}} & \quad\quad C(\thetav, \psiv) \label{eq:rate1} \\
\text{subject to} & \quad\quad \frac{1}{N}  \EE_{\xv}[E_A] = 1  \label{eq:rate2}\\
& \quad\quad \text{PAPR}_{\epsilon}(\thetav) = \gamma_{\text{peak}} \label{eq:rate3} \\
&  \quad\quad \text{ACLR}(\thetav) \leq \beta_{\text{leak}} \label{eq:rate4} 
 \end{align}
\end{subequations}
%
where \eqref{eq:rate2} ensures that the average energy per OFDM symbol equals $N$.

\subsection{System training}

%To deal with the problem \eqref{eq:rate}, we first formulate it as a constrained optimization problem following the framework presented in \cite[Chapter~3]{bertsekas2014constrained} and then solve it using the augmented Lagrangian method.
%In this section, we formulate the problem \eqref{eq:rate} as a constrained optimization problem that can be solved using the augmented Lagrangian method.
Solving the problem \eqref{eq:rate} is achieved by using the augmented Lagrangian method detailed in \cite[Chapter~3]{bertsekas2014constrained}.
This method converts the constrained optimization problem into its augmented Lagrangian that is minimized with respect to the trainable parameters $\thetav$ and $\psiv$.
Because the E2E system is composed of an \gls{NN}-based transmitter and receiver, their parameters can be optimized using \gls{SGD} as long as the loss function is differentiable. 
In this section, we therefore express the objective \eqref{eq:rate1} and the constraints \eqref{eq:rate3} and \eqref{eq:rate4} as differentiable functions that can be evaluated during training and minimized with \gls{SGD}.
The constraint \eqref{eq:rate2} is enforced with a normalization layer that is presented in the following.

To ensure a unitary mean energy per symbol, such normalization layer is added to the neural transmitter (see Fig.\ref{fig:system2}) and need to perform
%
\begin{align}
\label{eq:layer_norm*}
l_{\text{norm}}^*(\xv) = \frac{\xv}{ \left( \frac{1}{N} \EE_{\xv}[E_A] \right)^{\frac{1}{2}} } .
\end{align}
%
Computing the true value of $\EE_{\xv}[E_A]$ is of prohibitive complexity due to the $2^{KN}$ combinations of bits corresponding to different vectors $\xv$.
We therefore normalize each batch of transmitted signals to ensure it has an average energy of one. 
Each element $j$ of a batch is denoted by the superscript $[j]$ and is normalized as follows
%
\begin{align}
\label{eq:layer_norm}
l_{\text{norm}}(\xv^{[j]}) = \frac{\xv^{[j]}}{  \left( \frac{1}{N B_s}  \sum_{i=1}^{B_s}  \xv^{[i]^{\mathsf{H}}} \Wm \xv^{[i]} \right)^{\frac{1}{2}} }
\end{align}
%
%where the superscript $[i]$ denotes the $i^{\text{th}}$ element of the batch.
This expression accounts for the correlation that can appear  between the frequency baseband symbols generated by the neural transmitter.
Such correlation would not occur in conventional bit-interleaved coded modulation systems, as the baseband symbols would be independent and identically distributed.


%To minimize the augmented Lagrangian using \gsl{SGD}, the objective \eqref{eq:rate1} and the constraints \eqref{eq:rate2} to \eqref{eq:rate4} must be 
%To that aim, we express each training objectives \eqref{eq:rate1} to \eqref{eq:rate4} as loss functions that can be evaluated and minimized.
As derived in \cite{9118963}, maximizing the rate  of the communication system \eqref{eq:rate1} is equivalent to minimizing the total \gls{BCE}
%
\begin{align}
\label{eq:CE}
L_C(\thetav, \psiv) &:= - \frac{1}{N}\sum_{n=0}^{N-1}\sum_{k=0}^{K-1} \EE_{\yv} \left[ \text{log}_2 \left(\widehat{P}_{\psiv} (b_{n,k}| \yv ) \right) \right]  \\
& = K -  C(\thetav, \psiv). \nonumber
\end{align}
%
Because the exact computation of the \gls{BCE} value would be of prohibitive complexity, a common practice is to estimate it using Monte Carlo sampling with batches of size $B_s$:
\begin{align}
\label{eq:CE_batch}
L_C(\thetav, \psiv) \approx & - \frac{1}{NB_s}\sum_{n=0}^{N-1}\sum_{k=0}^{K-1}\sum_{i=0}^{B_s-1}  \text{log}_2 \left( \widehat{P}_{\psiv} \left( b_{n,k}^{[i]}| \yv ^{[i]} \right) \right).
\end{align}
%
%Finally, the rate of the transmission can be computed with \cite{9118963}
%%
%\begin{align}
%C(\thetav, \psiv) = K - L_C(\thetav, \psiv).
%\end{align}


The PAPR constraint \eqref{eq:rate3} can be interpreted as producing time-domain signals whose power $|s(t)|^2$ exceeds $\gamma_{\text{peak}}$ with a low probability.
However, evaluating \eqref{eq:papr} for arbitrary values of $\epsilon$ requires to count the amount of samples whose energy are higher than $\gamma_{\text{peak}}$, which is not differentiable.
%We therefore set $\epsilon=0$ during training and propose a constraint function that penalizes all signals exceeding the energy threshold:
We propose to substitute \eqref{eq:rate3} by a constraint function that penalizes all signals exceeding the threshold $\gamma_{\text{peak}}$, which is equivalent to setting $\epsilon=0$ :
%
\begin{align}
\label{eq:loss_papr}
L_{\gamma_{\text{peak}}}(\thetav)  = \EE \left[ \int_{-\frac{T}{2}}^{\frac{T}{2}} \text{max}\left(0, |s(t)|^2-\gamma_{\text{peak}} \right) dt \right].
\end{align}
%
Similarly to Section~\ref{sec:baseline}, let us denote by $\underline{\zv}  = \Fm^{-1}\xv \; \in \CC^{NO_s}$ the vector of discrete time signal oversampled with a factor $O_s$, where $\xv\in\CC^{N}$ is the output of the neural transmitter.
The expectation in \eqref{eq:loss_papr} can be approximated by sending a batch of signals, while the integral can be approximated using a Riemann sum, leading to
%
\begin{align}
L_{\gamma_{\text{peak}}}(\thetav)  \approx \frac{T}{B_s N O} \sum_{i=0}^{B_s-1} \sum_{t=-\frac{NO_s-1}{2}}^{\frac{NO_s-1}{2}} \text{max} \left(0, \left| \underline{z}_t^{[i]} \right| ^2 - \gamma_{\text{peak}} \right) .
\end{align}


Finally, inequality constraints such as \eqref{eq:rate4} can be converted to equality constraints using slack variables
$q\in\RR_+$:
%
\begin{align}
\text{ACLR} \leq \beta_{\text{leak}} \iff \text{ACLR} - \beta_{\text{leak}}  = -q .
\end{align}
%
This constraint can then be enforced my minimizing $L_{\beta_{\text{leak}}}(\thetav) + q $, with
%
\begin{align}
L_{\beta_{\text{leak}}}(\thetav)  & =  \frac{ \EE \left[ E_A \right]}{ \EE \left[ E_I \right]}-1   - \beta_{\text{leak}} \\
& \approx \frac{  \frac{1}{B_s} \sum_{i=0}^{B_s-1}  \xv^{[i]^{\mathsf{H}}} \Wm \xv^{[i]}}{ \frac{1}{B_s} \sum_{i=0}^{B_s-1}  \xv^{[i]^{\mathsf{H}}} \Vm \xv^{[i]}} -1   - \beta_{\text{leak}} .
\end{align}


%The problem \eqref{eq:rate} can now be expressed as the following constrained optimization problem:
The problem \eqref{eq:rate} can then be reformulated for $\epsilon = 0$ as the following constrained optimization problem:
%
\begin{subequations}
\label{eq:pb}
 \begin{align}
\underset{\thetav, \psiv}{\text{minimize}} & \quad\quad L_C(\thetav, \psiv) \label{eq:pb1} \\
\text{subject to} & \quad\quad L_{\gamma_{\text{peak}}}(\thetav)  = 0 \label{eq:pb2} \\
&  \quad\quad L_{\beta_{\text{leak}}}(\thetav) + q \leq 0 \label{eq:pb3} 
 \end{align}
\end{subequations}
%
%
for which the augmented Lagrangian is \cite[Chapter~3]{bertsekas2014constrained}
%
%\begin{align}
%\label{eq:lagrange_z}
%\overline{L} (\thetav, \psiv, z, \lambda_p, \lambda_l, & \mu_p, \mu_l)  = L_{C}(\thetav, \psiv) \nonumber \\
%& + \lambda_p L_{\gamma_{\text{peak}}}(\thetav) + \frac{1}{2}  \mu_p |L_{\gamma_{\text{peak}}}(\thetav)|^2 \\
%& + \lambda_l L_{\beta_{\text{leak}}}(\thetav) + z + \frac{1}{2} \mu_l | L_{\beta_{\text{leak}}}(\thetav) + z |^2 \nonumber
%\end{align}
\begin{align}
\label{eq:lagrange}
\overline{L} (\thetav, \psiv, \lambda_p, \lambda_l, & \mu_p, \mu_l)  = L_C(\thetav, \psiv) \nonumber \\
& + \lambda_p L_{\gamma_{\text{peak}}}(\thetav) + \frac{1}{2} \mu_p |L_{\gamma_{\text{peak}}}(\thetav)|^2 \\
& + \frac{1}{2\mu_l} \left( \text{max}(0, \lambda_l + \mu_l L_{\beta_{\text{leak}}}(\thetav) )^2 - \lambda_l^2 \right).  \nonumber
\end{align}
%
One can see that $q$ is not present in \eqref{eq:lagrange} since minimizing the augmented Lagrangian with respect to $q$ can be carried out explicitly for each fixed pair of $\{ \thetav, \psiv \}$ \cite{bertsekas2014constrained}.
The quantities $\mu_p > 0$ and $\mu_l>0$ are the penalty parameters and $\lambda_p, \lambda_l$ are the Lagrange multipliers for the constraint functions $L_{\gamma_{\text{peak}}}(\thetav)$ and $L_{\beta_{\text{leak}}}(\thetav)$ respectively.
%which replaces the original constrained problem by a sequence of unconstrained subproblems.
%As derived in \cite{bertsekas2014constrained}, minimizing $\overline{L} (\thetav, \psiv, z, \lambda_p, \lambda_l, \mu_p, \mu_l)$ with respect to $z$ can be carried out explicitly for each fixed pair of $\{ \thetav, \psiv \}$, and \eqref{eq:lagrange_z} can be simplified to
%
%\begin{align}
%\label{eq:lagrange}
%\overline{L} (\thetav, \psiv, \lambda_p, \lambda_l, & \mu_p, \mu_l)  = L_C(\thetav, \psiv) \nonumber \\
%& + \lambda_p L_{\gamma_{\text{peak}}}(\thetav) + \frac{1}{2} \mu_p |L_{\gamma_{\text{peak}}}(\thetav)|^2 \\
%& + \frac{1}{2\mu_l} \left( \text{max}(0, \lambda_l + \mu_l L_{\beta_{\text{leak}}}(\thetav) )^2 - \lambda_l^2 \right).  \nonumber
%\end{align}
%
The augmented Lagrangian method consists in iteratively minimizing \eqref{eq:lagrange}, each iteration comprising multiple steps of \gls{SGD}  followed by an update of the hyperparameters  $\lambda_p, \lambda_l, \mu_p$, and $\mu_l$.
The training procedure is described in Algorithm 1, where $\lambda_p^{(u)}, \lambda_l^{(u)}$, $\mu_p^{(u)}$, and $\mu_l^{(u)}$ denote the value of the hyperparameters at the $u^{\text{th}}$ iteration, and $\tau \in \RR_+$ controls the evolution of $\mu_p$ and $\mu_l$.
%
\begin{algorithm}
\label{algo}
\SetAlgoLined
 Initialize $\thetav, \psiv, \lambda_p^{(0)}, \lambda_l^{(0)}, \mu_p^{(0)}, \mu_l^{(0)}$ \\
 \For{$u = 0, ... $}{
  $\triangleright$ Perform multiple steps of SGD \\
  on $\overline{L} (\thetav, \psiv, \lambda, \lambda_l, \mu_p, \mu_l)$ w.r.t. $\thetav$ and $ \psiv$ \\
  $\triangleright$ Update optimization hyperparameters : \\
  $\lambda_p^{(u+1)} = \lambda_p^{(u)} + \mu_p^{(u)} L_{\gamma_{\text{peak}}}(\thetav) $\\
  $\lambda_l^{(u+1)} = \text{max} \left(0, \lambda_l^{(u)}  + \mu_l^{(u)} L_{\beta_{\text{leak}}}(\thetav) \right)$\\
  $\mu_p^{(u+1)} = (1+\tau) \mu_p^{(u)}$ \\
  $\mu_l^{(u+1)} = (1+\tau) \mu_l^{(u)}$ 
 }
 \caption{Training procedure}
\end{algorithm}


%\begin{algorithm}
%\label{algo}
%\SetAlgoLined
% Initialize $\thetav, \psiv, \lambda_p^{(0)}, \lambda_l^{(0)}, \mu_p^{(0)}, \mu_l^{(0)}$ \\
% \For{$u = 0, ... $}{
%  $\triangleright$ Perform multiple steps of SGD \\ 
%  on $\overline{L} (\thetav, \psiv, \lambda, \lambda_l, \mu_p, \mu_l)$ \\
%  $\triangleright$ Update optimization parameters : \\
%  $\lambda_p^{(u+1)} = \lambda_p^{(u)} + \mu_p^{(u)} L_{\gamma_{\text{peak}}}(\thetav) $\\
%  $\lambda_l^{(u+1)} = \text{max} \left(0, \lambda_l^{(u)}  + \mu_l^{(u) L_{\beta_{\text{leak}}}(\thetav) \right)$\\
%  $\mu_p^{(u+1)} = (1+\epsilon) \mu_p^{(u)}$ \\
%  $\mu_l^{(u+1)} = (1+\epsilon) \mu_l^{(u)}$ 
% }
% \caption{Training procedure}
%\end{algorithm}

\subsection{System architecture}

%\begin{figure}[t]
%    \centering
%    \includegraphics[height=85pt]{figs/resnet_h.png}
%    \caption{Architecture of a ResNet Block}
%    \label{fig:resnet_h}
%\end{figure}



\begin{figure}
\centering
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[height=125pt]{figs/resnet.png}
  \caption{ResNet block.}
  \label{fig:resnet_h}
\end{subfigure}%
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[height=125pt]{figs/NN_Tx.png}
  \caption{NN-Transmiter.}
  \label{fig:nn_tx_h}
\end{subfigure}
\begin{subfigure}{.16\textwidth}
  \centering
  \includegraphics[height=125pt]{figs/NN_Rx.png}
  \caption{NN-Receiver.}
  \label{fig:nn_rx_h}
\end{subfigure}%
\caption{Different parts of the end-to-end system, where grayed blocks are trainable components. The IDFT/DFT operations and the channel are not represented for clarity.}
\label{fig:components}
\end{figure}



Both the \gls{NN}-based transmitter and receiver use ResNet blocks, originally presented in \cite{he2016identity}, and which were proven to be effective in physical layer tasks \cite{honkala2020deeprx, pilotless20, 9460758}.
A ResNet block is composed of a residual connection preceded by two groups of layers, each containing a batch normalization layer, a ReLU, and a 1D separable convolution (Fig. \ref{fig:resnet_h}). 
Such a convolution maintains similar performance compared to a traditional convolution while being less computationally demanding \cite{howard2017mobilenets}.
All 1D separable convolutions use zero-padding to maintain the first dimension of constant size.

The neural transmitter (Fig. \ref{fig:nn_tx_h}) is composed of two convolutional layers, multiple ResNet blocks, a layer that converts $2N$ real numbers to $N$ complex numbers, and a normalization layer as expressed in \eqref{eq:layer_norm}.
The sequence of trainable layers forms a \gls{CNN}, which takes as input the matrix of bits $\Bm\in\{0,1\}^{N \times K}$, where $N$ corresponds to the 1D convolution dimension and $K$ to the number of input channels.
The last separable convolution has only two filters such that the output, of dimension $N\times 2$, can be converted to the baseband frequency symbols $\xv \in \CC^N$.

The neural receiver, depicted in Fig. \ref{fig:nn_rx_h}, uses a similar architecture.
The signal $\yv$ is first converted to a matrix of dimension $N \times 2$, which is processed by the \gls{CNN} as two different channels of dimension $N$.
The last separable convolution has $K$ filters, corresponding to the $K$ \glspl{LLR} that need to be predicted for every symbol. 
The exact parameters of each trainable component are listed in the next section.

%\begin{figure}[t]
%    \centering
%    \includegraphics[height=85pt]{figs/nn_tx_h.png}
%    \caption{Architecture of the neural transmitter.}
%    \label{fig:nn_tx_h}
%\end{figure}
%
%\begin{figure}[t]
%    \centering
%    \includegraphics[height=85pt]{figs/nn_rx_h.png}
%    \caption{Architecture of the neural receiver.}
%    \label{fig:nn_rx_h}
%\end{figure}


==> V1/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


We have presented an E2E system that can be optimized to maximize an achievable information rate while satisfying constraints on the signal PAPR and ACLR.
The optimization objective and the two constraints were expressed as differentiable functions that can be minimized using \gls{SGD}.
The constrained optimization problem was solved using the augmented Lagrangian method, where the corresponding augmented Lagrangian is minimized iteratively.
Numerical results demonstrated the effectiveness of the proposed approach, with trained systems that meet ACLR and PAPR targets while achieving rates comparatively higher than the baseline.
This work can be seen as a first step towards learning of new waveforms for future generations of ACLR- and PAPR-constrained systems.
Scaling to more subcarriers and the integration of more realistic channels constitute possible research directions.

%\flushend 

==> V1/sections/experiments.tex <==
\section{Evaluations} 
\label{sec:evaluations}

\subsection{Setup}
\label{sec:evaluation_setup}

\begin{table}

\centering

\newcolumntype{M}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{N}{@{}m{0pt}@{}}

\renewcommand{\arraystretch}{2}

\begin{tabular}{ |M{1.3cm}||M{0.7cm}|M{0.45cm}|M{0.45cm}|M{0.45cm}|M{0.45cm}|M{0.45cm}|M{0.7cm}| N }
 \hline
 	& Sep. Conv. & \multicolumn{5}{c|}{ResNet blocks} & Sep. Conv \\
 \hline
 Kernel size & 1 & 3 & 9 & 15 & 9 & 3 & 1\\
 \hline
 Dilation rate & 1 & 1 & 2 & 4 & 2 & 1& 1\\
 \hline
 \# Filters & \multicolumn{7}{c|}{128}\\
 \hline
\end{tabular}

\caption{Parameters for the \gls{CNN} transmitter and receiver.}
\label{table}
\renewcommand{\arraystretch}{1}

\end{table}

\begin{figure}[t]
\input{figs/rates_papr_2.tex}
\caption{Rates achieved by the baseline and two E2E systems. The numbers represent the corresponding ACLRs.}
\label{fig:rates}
%\vspace{-2pt}
\end{figure}

\begin{figure}[t]
\input{figs/CCDF_2.tex}
\caption{CCDF of the signal power for two systems having similar rates.}
\label{fig:ccdf}
%\vspace{-8pt}
\end{figure}

\begin{figure}[t]
\input{figs/PSD_smooth.tex}
\caption{PSD of three systems with similar PAPRs.}
\label{fig:psd}
\end{figure}

To evaluate the proposed scheme, an \gls{OFDM} system with $N=75$ subcarriers and an \gls{AWGN} channel is considered.
The \gls{SNR} of the transmission is set to 10~\si{dB}, both during training and evaluation.
%The number of subcarriers is kept relatively small in order to enable fast convergence during training, but some standards use even lower numbers.
%For example, the IEEE 802.11a specification only uses 52 subcarriers, while the more recent 802.11ac specification uses between 64 and 512 subcarriers.
The number of bits per channel use is set to $K=4$, and the baseline uses 16-QAM.

The transmitter and receiver share the same \gls{CNN} architecture, whose parameters are listed in Table \ref{table}.
It is worth noting that dilations are used to increase the receptive field of the \glspl{CNN}.
The optimization parameters are initialized at $\lambda_p^{(0)}=0, \lambda_l^{(0)}=0, \mu_p^{(0)}=0.1$, and $\mu_l^{(0)}=0.001$, and $\tau$ is set to $0.004$.
The difference in initialization between $\mu_p^{(0)}$ and $\mu_l^{(0)}$ reflects the fact that $L_{\beta_{\text{leak}}}(\thetav)$ is usually two orders of magnitude higher than  $L_{\gamma_{\text{peak}}}(\thetav)$.
The training process is composed of 2500 iterations, each including 15 \gls{SGD} steps are performed with a batch size of $B_s=1500$.
%At the end of the training sequence, the penalty parameters reach respectively $\mu_p^{(2500)}\approx 2000$ and $\mu_l^{(2500)}\approx 20$, which was sufficient to be close to the target ACLRs and PAPRs.
During training, $L_{\gamma_{\text{peak}}}(\thetav)$ is approximated using a temporal oversampling factor of $O_s=5$, which was found to be enough to accurately represent the continuous analog waveform \cite{922754}.
The baseline is evaluated for  $R \in \{0, 2, 4, 8, 16\}$ \glspl{PRT}, and the E2E system is trained for $\gamma_{\text{peak}} \in \{ 4, 5, 6, 7, 8, 9\}$~\si{dB} and two ACLR targets: $\beta_{\text{leak}}=-20$~\si{dB}, which corresponds to the baseline ACLR, and $\beta_{\text{leak}}=-30$~\si{dB}.




\subsection{Results}



In the following evaluations, the target \gls{PAPR} probability threshold in \eqref{eq:papr} is set to $\epsilon=10^{-3}$.
This is different from the value used for training, which was set to  $\epsilon=0$ in order to define a differentiable cost function.
Fig. \ref{fig:rates} shows the rates and \glspl{PAPR} achieved by the baseline and the two systems trained with target ACLRs of -20~\si{dB} and -30~\si{dB}.
The numbers next to the plots represent the \glspl{ACLR} of each evaluated system.
Firstly, it can be seen that all E2E systems satisfy the \gls{ACLR} targets. 
%Secondly, the systems trained with $\beta_{\text{leak}} = -20$~\si{dB} achieves higher rates than the systems trained with $\beta_{\text{leak}} = -30$~\si{dB}.
Secondly, for PAPRs lower than 7~\si{dB}, both trained systems achieve higher rates than the baseline, which is particularly interesting since the second system also achieves a 10~\si{dB} lower ACLR.
For PAPRs higher than 7.5~\si{dB}, the baseline and the system trained with $\beta_{\text{leak}} = -20$~\si{dB} enable similar performance.
Finally, it can be seen that the the training procedure allows to control the PAPR of the transmission.
Lower PAPR thresholds $\epsilon < 10^{-3}$ could be enforced by choosing a higher scalar $\tau$ during training. 
%Indeed, at low PAPRs, the largest difference between the target and the effective PAPR is of 0.35 for the system trained with $\gamma_{\text{peak}} = 4$ and $\beta_{\text{leak}} = -30$~\si{dB}.
%At high PAPRs, all trained scheme achieve slightly lower PAPRs than their respective targets.
%These results tends to confirm the effectiveness of the proposed training procedure, as the \gls{ACLR} constraints are satisfied and the \glspl{PAPR} are close to the target ones.




To visualize the effect of the \gls{PAPR} reduction on the signal energy, the \gls{CCDF} of two systems having similar rates are shown in Fig.\ref{fig:ccdf}.
These two systems are the baseline with 2 PRTs and the E2E system trained with $\gamma_{\text{peak}} = 6$~\si{dB} and $ \beta_{\text{leak}} = -20$~\si{dB},  respectively represented with a black square and a red circle in Fig. \ref{fig:rates}.
The \gls{CCDF} of the signal energy is expressed as
%
\begin{align}
\text{CCDF}_{|s(t)|^2}(x) = P \left( |s(t)|^2 > x \right).
\end{align}
%
It can be seen that the CCDF of the E2E system is significantly lower than the one of the baseline, which results in a difference of approximately 1.4~\si{dB} at a CCDF of $10^{-3}$.



Finally, the power spectral densities (PSDs) of three systems are shown in Fig.~\ref{fig:psd}.
The first one is the baseline with no \glspl{PRT}.
The second and third ones are E2E systems trained with the highest PAPR constraint ($\gamma_{\text{peak}}=9$~\si{dB}) and ACLR constraints respectively set to $\beta_{\text{leak}}=-20$~\si{dB} and $\beta_{\text{leak}}=-30$~\si{dB}.
It can be observed that the PSD of the baseline and that of the system trained with $\beta_{\text{leak}}=-20$~\si{dB} are nearly identical, but the PSD of the system trained with $\beta_{\text{leak}}=-30$~\si{dB} has considerably less out-of-band energy.


==> V1/sections/introduction.tex <==
\section{Introduction} 
\label{sec:introduction}

With the ever-growing demand for services that depend on radio connectivity, future wireless systems will need to satisfy increasingly difficult requirements on the signal characteristics.
Due to its low complexity implementation, \gls{OFDM} is used in many modern communication systems and is a potential candidate waveform for the next generation of wireless networks.
However, when used in conjunction with conventional \gls{QAM}, the generated signal exhibits both low spectral containment and high \gls{PAPR}.
%
%On the one hand, the \gls{ACLR} might prevent \gls{OFDM} systems to be used in specific frequency-constrained environments.
The \gls{ACLR} of \gls{OFDM} waveforms is typically decreased by the introduction of guard subcarriers at the cost of a reduced spectral efficiency.
High \glspl{PAPR} either leads to distortions of the transmitted signal or to the use of high power backoffs, reducing the \gls{PA} efficiency.
%The high signal amplitudes imply that the signal power often lies in the \gls{PA} saturation region.
%This either signifies that the amplified signal will suffers from important distortions or that the \gls{PA} will be operated with a power back-off, thus reducing the energy efficiency of the system.

Multiple techniques have been proposed to reduce the \gls{PAPR} of \gls{OFDM} signals, such as clipping and filtering \cite{wang2010optimized}, constellation extension \cite{krongold2003reduction}, and tone reservation \cite{1261335}.
The latter approach uses a subset of the available subcarriers to create a peak-canceling signal, and was recently combined with deep \glspl{NN} to predict the peak-canceling signal from the frequency baseband symbols to be transmitted~\mbox{\cite{wang2020novel, wang2021model, 8928103}}.
%
In~\cite{8240644}, it has been proposed to treat the communication system as an autoencoder, where the transmitter and receiver are trained to jointly minimize the \gls{BER} and \gls{PAPR} of the transmission.
Although the presented autoencoder shows promising results, the \gls{PAPR} is minimized based on a non-oversampled time-discrete signal, which is not fully representative of its  analog waveform \cite{1261335}.
Moreover, the autoencoder operates on symbols, meaning that \gls{QAM} mapping and demapping are still required.
Finally, none of these previous works allow to define target values for the PAPR and ACLR, and therefore to control the tradeoff between the spectral efficiency and the PAPR and ACLR requirements.

%In this work, we propose to learn new high-dimensional symbol mappings and corresponding demappings using a training procedure that maximizes the information rate of the transmission while satisfying any \gls{PAPR} and \gls{ACLR} constraints.
%The main idea is to formulate the training objective as a constrained optimization problem, which is then solved iteratively through minimizing an equivalent sequence of unconstrained subproblems.
%%
%To do so, the rate, \gls{ACLR} and \gls{PAPR} expressions are first converted into loss functions that can be approximated and minimized.
%The constrained optimization problem is then expressed as an \emph{augmented Lagrangian}, which is a combination of these loss functions with specific optimization parameters.
%Finally, the augmented Lagrangian is minimized by iterating between multiple step of \gls{SGD} and optimization parameters updates.

In this work, we propose to jointly optimize an \gls{NN}-based high-dimensional modulation scheme on the transmitter side and an NN-based detector on the receiver side, that operate on top of OFDM. % and a channel model.
The end-to-end system is trained to maximize an achievable information rate, while satisfying constraints on the ACLR and PAPR. 
The key idea is to formulate the training objectives as a constrained optimization problem, which is then solved iteratively using the augmented Lagrangian method.
To that aim, the achievable rate, \gls{ACLR}, and \gls{PAPR} of the transmission are expressed as functions that can be evaluated during training and minimized using \gls{SGD}.
%To that aim, a constrained optimization problem is formulated, which is then solved using the augmented Lagrangian method.
%To to so, the rate, \gls{ACLR}, and \gls{PAPR} of the transmission are expressed as loss functions that can be approximated and minimized using \gls{SGD}.
%
Evaluations show that the end-to-end system achieves competitive or higher rates compared to a \gls{TR} baseline, while having similar or lower ACLRs and PAPRs.
As an example, the trained system outperforms the \gls{TR} baseline while having a 0.7~\si{dB} and 10~\si{dB} reduced PAPR and ACLR, respectively.
%With a similar \gls{ACLR}, the trained systems generate signals that satisfy the \gls{PAPR} constraints while matching or exceeding the transmission rate of the corresponding baseline.
%When trained for an \gls{ACLR} 10~\si{dB} lower than the baseline, the trained systems are still able to outperform the baseline for target \glspl{PAPR} lower than 7~\si{dB}.
%
%As an example, the end-to-end system achieves up to X higher rates, despite enabling ACLR and PAPR 10dB and 7dB lower, respectively, when compared to a PRT baseline.

%\textbf{Notations :} 
%Matrices and column vectors are respectively denoted by bold upper- and lower-case letters. 
%$x_{i}$ is the $i^{\text{th}}$ element of the vector $\xv$, and $x_{i,j}$ the $(i,j)^{\text{th}}$ element of the matrix $\Xm$.
%$(\cdot)\htp$ denotes the conjugate transpose operator, and $\Vert \cdot \Vert_{\infty}$ is the infinity norm.
%Finally, $j$ is the imaginary unit such that $j^2 = -1$.




==> V1/sections/ml_enhanced.tex <==
\section{End-to-End Trainable system}
\label{sec:autoencoder}






==> V1/sections/problem_positioning.tex <==
\section{Problem positioning} 
\label{sec:problem_positioning}



\subsection{System model}
\label{sec:system_model}

An \gls{OFDM} system with $N$ subcarriers is considered, the subcarriers being indexed by the set $\mathcal{N}= \{ -\frac{N-1}{2}, \dots, \frac{N-1}{2} \}$, where $N$ is assumed to be odd for convenience.
The matrix of bits to be transmitted is denoted by $\Bm = \left[ \bv_1, \dots, \bv_N \right]\tp$, where $\bv_{n\in\mathcal{N}} \in \{0, 1\}^{K}$ are the vectors of bits to be sent and $K$ is the number of bits per channel uses.
$\Bm$ is modulated onto discrete baseband symbols $\xv \in \CC^{N}$ that are mapped on the orthogonal subcarriers, forming the baseband spectrum
%
\begin{equation}
\begin{split}
S(f) & = \sum_{n=-\frac{N-1}{2}}^{\frac{N-1}{2}} x_n \frac{1}{\sqrt{\Delta_f}} \text{sinc} \left( \frac{f}{\Delta_f} - n \right) . \\
\end{split}
\end{equation}
where $\Delta_f$ is the subcarrier spacing.
The corresponding time-domain signal, of duration $T=\frac{1}{\Delta_f}$, is
%
\begin{equation}
\begin{split}
s(t) & = \sum_{n=-\frac{N-1}{2}}^{\frac{N-1}{2}} x_n \frac{1}{\sqrt{T}} \text{rect} \left( \frac{t}{T} \right) e^{i 2 \pi n t/T}  \\
\end{split}
\end{equation}
%
where $t \in [-\frac{T}{2}, \frac{T}{2}]$. 
%In the following, all discrete baseband symbols will be normalized such that $\EE \left[|s(t)|^2 \right] = 1$.

A major limitation of \gls{OFDM} is its high PAPR, which either implies that the output signal might suffer from distortions due to the \gls{PA} saturation, or that the \gls{PA} must be operated with a large power back-off, reducing its power efficiency \footnote{A  substantial power backoff is required although \gls{DPD} is widely used to reduce the detrimental effect of such distortions.}.
In the following, we define the \gls{PAPR} of a signal as the smallest threshold $e \geq 0$, such that the probability of the ratio between the instantaneous and average squared signal amplitude being larger than that $e$ is smaller than a threshold $\epsilon\in(0,1)$:
%the minimum energy $e$ above which the instantaneous signal energy $|s(t)|^2$ lies with a small probability  $\epsilon \in (0, 1)$, i.e., 
%
\begin{equation}
\label{eq:papr}
\begin{split}
\text{PAPR}_{\epsilon}  \coloneqq \mathrm{min} \; e, \;\; \text{s. t.} \;\;  P\left( \frac{|s(t)|^2}{\EE \left[|s(t)|^2 \right]} > e  \right) \leq \epsilon.
\end{split}
\end{equation}
%
%\begin{equation}
%\begin{split}
%\text{PAPR} & = \gamma  \; s.t. \; P \left( 10 \text{log}_{10} \left(|s(t)|^2 \right) > \gamma \right) = 10^{-2}.\\
%\end{split}
%\end{equation}
We do not use the more conventional definition $ \frac{\max{|s(t)|^2}}{\EE \left[|s(t)|^2 \right]}$, as it only considers the max signal amplitude and is therefore less representative of the overall power distribution.

To quantify the spectral containment of waveforms, one typically uses the \gls{ACLR}, which is defined as the ratio between the expected out-of-band energy $\EE_{\xv} \left[ E_O\right]$ and the expected in-band energy $\EE_{\xv} \left[ E_I\right]$ :
\begin{equation}
\begin{split}
\text{ACLR} & \coloneqq  \frac{\EE_{\xv} \left[ E_O\right]}{\EE_{\xv} \left[ E_I\right]} 
 =   \frac{\EE_{\xv} \left[ E_A \right]}{\EE_{\xv} \left[ E_I \right]}-1 \\
\end{split}
\end{equation}
where $E_A = E_O + E_I $ is the total energy of the transmitted signal.
%Let us denote $\xv \in \CC^{N} = \left[ X[-\frac{N-1}{2}], \dots, X[\frac{N-1}{2}] \right]$ the vector of frequency symbols to be transmitted.
% and $\sv \in \CC^{N} = \text{IDFT}(\xv)$ their corresponding time-domain samples.
The in-band energy $E_I$ is
%
\begin{equation}
\begin{split}
E_{I} & \coloneqq \int_{-\frac{N \Delta_f}{2}}^{\frac{N \Delta_f}{2}} \left| S (f)\right|^2 df = \xv ^H \Vm \xv, \\
\end{split} 
\end{equation}
where each element $v_{a, b}$ of the matrix $\Vm$ is 
\begin{equation}
v_{a, b} = \frac{1}{\Delta_f} \int_{-\frac{N \Delta_f}{2}}^{\frac{N \Delta_f}{2}}  \text{sinc} \left(\frac{f}{\Delta_f}-a \right) \text{sinc} \left(\frac{f}{\Delta_f}-b \right) df.
\end{equation}
%
The total transmitted energy can be similarly computed in the time domain :
\begin{equation}
\begin{split}
E_{A} & \coloneqq \int_{ -\frac{T}{2}}^{\frac{T}{2}} \left| s (t)\right|^2 dt = \xv ^H \Wm \xv, \\
\end{split} 
\end{equation}
where $\Wm$ is such that 
\begin{equation}
w_{a, b} = \frac{1}{T} \int_{-\frac{T}{2}}^{\frac{T}{2}}  e^{i 2 \pi (a-b) t /T} dt .
\end{equation}
In the following, an \gls{AWGN} channel is considered, and the vector of received baseband symbols is denoted by $\yv \in \CC^{N}$.


\subsection{Baseline}
\label{sec:baseline}

One technique to reduce the \gls{PAPR} of \gls{OFDM} signals is tone reservation (TR), in which a subset of $R$ subcarriers (tones) are used as \glspl{PRT}.
These tones do not carry data, but are used to minimize the peak amplitude of the time-domain signal.
The set of all \glspl{PRT} is denoted by $\mathcal{R} \subset \mathcal{N}$, and the set containing the remaining $D$ subcarrier used for data transmission is denoted by $\mathcal{D} \subseteq \mathcal{N} $, with $\mathcal{D} \cup \mathcal{R} = \mathcal{N}$.
The vector of signals mapped to the \glspl{PRT} is referred to as the reduction signal $\cv\in\CC^{N}$, and $\xv$ and $\cv$ are such that $x_{n\in \mathcal{R}} = 0$ and $c_{n\in \mathcal{D}} = 0 $.
The vector of transmitted baseband symbols is denoted by $\xv' = \xv + \cv$.


\begin{figure}
\input{figs/waveform.tex}
\caption{OFDM signal generated from $N=75$ subcarriers.}
\label{fig:waveform}
%\vspace{-5pt}
\end{figure}

The corresponding continuous-time signal is denoted by $s'(t)$ and minimizing its PAPR amounts to finding 
%
\begin{equation}
\label{eq:c_star}
\begin{split}
\arg\min_{\cv} \max_{t} |s'(t)|^2.
\end{split}
\end{equation}
%

In practice, minimization cannot be performed directly on the time-continuous signal, and $s'(t)$ must therefore be discretized.
Many previous works only consider a non-oversampled discrete signal to represent the analog waveform~{\cite{wang2021model, 8928103, 8240644}}.
However, it has been shown that oversampling is necessary to correctly represent the underlying continuous signal \cite{1261335}.
Let us denote by $\zv\in\CC^N$ and $\underline{\zv}\in\CC^{NO_s}$ the signal sampled with a period $\frac{T}{N}$ and the signal oversampled by a factor $O_s$, respectively.
The difference between them is illustrated in Fig.~\ref{fig:waveform}, where the time-domain signal of an OFDM symbol is represented with and without oversampling ($O_s=5$ in this example).
%
First, it can be observed that the two signals have very different power peaks, indicated by dashed lines.
Second, $\underline{\zv}$ shows many more secondary peaks, which might lie in the \gls{PA} saturation region and therefore must be considered when reducing the signal distortion.
This oversampled signal can be obtained by computing the inverse discrete Fourier transform (IDFT) of $\xv'$ with adequate \mbox{zero-padding :}
\begin{equation}
\underline{\zv} = \Fm^{-1} (\xv + \cv),
\end{equation}
where $\Fm^{-1}\in\CC^{NO \times N}$ is the corresponding IDFT matrix.
%

The problem \eqref{eq:c_star} can be approximated by minimizing on the oversampled signal, i.e., 
%
\begin{equation}
\label{eq:convex_min}
  \arg\min_{\cv} \left\Vert g\left(\Fm^{-1} (\xv + \cv)\right)  \right\Vert_{\infty}
\end{equation}
where $g(\cdot)$ computes the element-wise squared magnitude $|\cdot|^2$.
%
Numerous iterative algorithms have been proposed to approximately solve \eqref{eq:convex_min} (see, e.g., \cite{1261335}). 
As the function \mbox{$h(\xv')= \left\Vert g\left(\Fm^{-1} (\xv')\right)  \right\Vert_{\infty}$} is convex, we use a convex solver~\cite{diamond2016cvxpy} to solve \eqref{eq:convex_min} for each vector of symbols $\xv$.
Moreover, it was shown that placing PRTs at randomly sampled locations at each transmission leads to the lowest PAPR~\mbox{\cite{peterssonPAPR, 1261335}}.
We therefore used such a random PRT allocation as baseline.
Note that neither using a convex solver nor a random PRT allocation is practical because of the incurred complexity and overhead required to indicate the \glspl{PRT} positions to the receiver.
However, it was considered for benchmarking our approach as it provides the lowest PAPR.




%Numerous techniques have been proposed to approximate $\cv^*$ in a finite number of iterations \cite{1261335}, but as the function  $h(\xv')= \left\Vert g\left(\Fm^{-1} (\xv')\right)  \right\Vert_{\infty}$ is convex, the baseline leverages tone reduction with $\cv^*$ computed from convex optimization on the discretized oversampled signal.
%Our experiments, supported by other existing works \cite{peterssonPAPR, 1261335}, indicates that placing the \glspl{PRT} at random location yields lower \glspl{PAPR} than other placement techniques.
%Therefore, the elements of $\mathcal{R}$ are chosen randomly in $\mathcal{N}$ for every transmissions.




Aside from leveraging \gls{TR}, the baseline uses a conventional \gls{QAM} modulation to map each vector of bits $\bv_{n\in\mathcal{D}}$ to a baseband symbol $x_{n\in\mathcal{D}}$.
These symbols are then transmitted using an OFDM waveform.
Because an \gls{AWGN} channel is considered, the receiver recovers the baseband symbols $\yv$ by performing a DFT on the subcarriers $n\in{\mathcal{D}}$.
The \glspl{LLR} are then computed using a standard \gls{AWGN} demapper.














==> sections/ml_enhanced.tex <==
\section{End-to-End Trainable system}
\label{sec:autoencoder}





